Towards Fine-Grained Information: Identifying the Type and Location of Translation Errors

Fine-grained information on translation errors is helpful for the translation evaluation community. Existing approaches can not synchronously consider error position and type, failing to integrate the error information of both. In this paper, we propose Fine-Grained Translation Error Detection (FG-TED) task, aiming at identifying both the position and the type of translation errors on given source-hypothesis sentence pairs. Besides, we build an FG-TED model to predict the \textbf{addition} and \textbf{omission} errors -- two typical translation accuracy errors. First, we use a word-level classification paradigm to form our model and use the shortcut learning reduction to relieve the influence of monolingual features. Besides, we construct synthetic datasets for model training, and relieve the disagreement of data labeling in authoritative datasets, making the experimental benchmark concordant. Experiments show that our model can identify both error type and position concurrently, and gives state-of-the-art results on the restored dataset. Our model also delivers more reliable predictions on low-resource and transfer scenarios than existing baselines. The related datasets and the source code will be released in the future.

==> table_example.tex <==
\begin{CJK}{UTF8}{gbsn}
\begin{table*}[htbp]
    \centering
    \small
    \scalebox{1.0}{
    \begin{tabular}{llcc}
            \toprule
            & & \textbf{\textsc{Src}} & \textbf{\textsc{Hyp}} \\
            \midrule
            \multicolumn{2}{c}{\textbf{Original}} & 学校和幼儿园开学了。 & Schools were opened yesterday. \\
            \cdashline{1-4}[1pt/2.5pt]\noalign{\vskip 0.5ex}
            \multirow{2}{*}{\textbf{Error}} &
            Addition & 学校和幼儿园开学了。 & Schools were opened \textcolor{red}{yesterday}. \\
            & Omission & 学校\textcolor{cyan}{和幼儿园}开学了。 & Schools were opened yesterday.\\
            
            \bottomrule
             
        \end{tabular}
    }
    \caption{A toy illustration of our task. The first line gives the original source and a machine translation hypothesis. While the second line and the third line give the \textcolor{red}{addition error} and the \textcolor{cyan}{mission error} for this hypothesis, respectively.}
    \label{table_example}
\end{table*}
\end{CJK}

==> table_task.tex <==

\begin{table}[t]
    \centering
    \small
    \scalebox{0.6}{
    \begin{tabular}{lcccc}
            \toprule
            Task & Error Position & Error Type &  Unsupervise & word-level\\
            \midrule
            Ours & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
            Word-level QE & \ding{51} & \ding{55} & \ding{55} & \ding{51} \\
            Critical Error Detection (CED) & \ding{55} & \ding{51} & \ding{55} & \ding{55}\\
            \bottomrule
        \end{tabular}
    }
    \caption{This table describes how our task differs from other fine-grained translation evaluation tasks. Our task can be seen as a combination of previous fine-grained translation evaluation tasks.}
    \label{table.task}
\end{table}

